Pillar-0: A New Frontier for Radiology Foundation Models

Radiology plays an integral role in modern medicine, yet rising imaging volumes have far outpaced workforce growth. Foundation models offer a path toward assisting with the full spectrum of radiology tasks, but existing medical models remain limited: they process volumetric CT and MRI as low-fidelity 2D slices, discard critical grayscale contrast information, and lack evaluation frameworks that reflect real clinical practice. We introduce Pillar-0, a radiology foundation model pretrained on 42,990 abdomen-pelvis CTs, 86,411 chest CTs, 14,348 head CTs, and 11,543 breast MRIs from a large academic center, together with RATE, a scalable framework that extracts structured labels for 366 radiologic findings with near-perfect accuracy using LLMs. Across internal test sets of 14,230 abdomen-pelvis CTs, 10,646 chest CTs, 4,906 head CTs, and 1,585 breast MRIs, Pillar-0 establishes a new performance frontier, achieving mean AUROCs of 86.4, 88.0, 90.1, and 82.9, outperforming MedGemma (Google), MedImageInsight (Microsoft), Lingshu (Alibaba), and Merlin (Stanford) by 7.8-15.8 AUROC points and ranking best in 87.2\% (319/366) tasks. Pillar-0 similarly outperforms all baselines in an external validation on the Stanford Abdominal CT dataset, including Merlin (82.2 vs 80.6 AUROC). Pillar-0 extends to tasks beyond its pretraining, such as long-horizon lung cancer risk prediction, where it improves upon the state-of-the-art Sybil by 3.0 C-index points on NLST, and generalizes with gains of 5.9 (MGH) and 1.9 (CGMH). In brain hemorrhage detection, Pillar-0 obtained a >95 AUROC when using only 1/20th of the data of the next most sample efficient baseline. Pillar-0 and RATE together provide an open, clinically rigorous foundation for building high-performance radiology systems, enabling applications that were previously infeasible due to computational, data, and evaluation constraints.

==> results/misc.tex <==


% THESE ARE THE TABLES WHICH ARE PART OF FIGURES 3 AND 4


% \begin{table}[t]
% \centering
% % \caption{Evaluation Frameworks}
% \label{tab:benchmark_characteristics}
% \begin{tabularx}{\linewidth}{l *{5}{>{\centering\arraybackslash}X}}
% \toprule
% \textbf{Evaluation Framework} &
% \textbf{Full-resolution volume inputs} &
% \textbf{Tasks and labels derived from real-world data} &
% \textbf{Extensible to new hospital data} \\
% \midrule
% VQA-RAD & \n & \n & \n\\
% SLAKE &\n & \n & \n \\
% PMC-VQA & \n & \n &  \n \\
% OmniMedVQA & \n & \n \\
% MMMU & \n & \n & \n \\
% RadLE & \n & \y & \n \\
% MedXpertQA & \n & \n & \n \\
% \midrule
% \textbf{RATE (Ours)} & \y & \y & \y\\
% \bottomrule
% \end{tabularx}
% \end{table}

% \begin{table}[t]
% \centering
% % \caption{Evaluation Frameworks}
% \label{tab:benchmark_characteristics}
% \begin{tabularx}{\linewidth}{l *{5}{>{\centering\arraybackslash}X}}
% \toprule
% \textbf{Evaluation Framework} &
% \textbf{Full-resolution volume inputs} &
% \textbf{Tasks and labels derived from real-world data} &
% \textbf{Extensible to new hospital data} \\
% \midrule
% VQA-RAD & \n & \n & \n\\
% SLAKE &\n & \n & \n \\
% PMC-VQA & \n & \n &  \n \\
% OmniMedVQA & \n & \n \\
% MMMU & \n & \n & \n \\
% RadLE & \n & \y & \n \\
% MedXpertQA & \n & \n & \n \\
% \midrule
% \textbf{RATE (Ours)} & \y & \y & \y\\
% \bottomrule
% \end{tabularx}
% \end{table}

% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \begin{table}[t]
% \centering
% % \caption{Evaluation Frameworks}
% \label{tab:benchmark_characteristics}
% % \begin{tabularx}{\linewidth}{l *{5}{>{\centering\arraybackslash}X}}
% \begin{tabularx}{\linewidth}{p{0.2\linewidth} C{0.15\linewidth} C{0.33\linewidth} C{0.2\linewidth}}
% \toprule
% \textbf{Evaluation Framework} &
% \textbf{Inputs} &
% \textbf{Task and label source} &
% \textbf{Extensibility} \\
% \midrule
% VQA-RAD & 2D slices & Medical student QA & \n\\
% SLAKE & 2D slices & Physician QA with knowledge graph-curated labels & \n \\
% PMC-VQA & 2D slices & Medical figures and captions & \n \\
% OmniMedVQA & 2D slices & Classification datasets & \n \\
% MMMU & 2D slices & Textbooks, online resources & \n \\
% RadLE & 2D slices & Radiologist-selected complex cases & \n \\
% MedXpertQA & 2D slices & Medical exams and textbooks & \n \\
% \midrule
% \textbf{RATE (Ours)} & \textbf{Full-resolution 3D volumes} & \textbf{Real-world radiology workflows} & \textbf{Can be extended to any new dataset} \\
% \bottomrule
% \end{tabularx}
% \end{table}

% \newcolumntype{L}{l<{\hspace{1.5em}}}

% \begin{table}[htbp]
% \centering
% \caption{Baselines}
% \label{tab:baselines}
% \begin{tabularx}{\linewidth}{L c c c >{\raggedright\arraybackslash}X}
% \toprule
% \textbf{Model} &
% \textbf{Model size} &
% \textbf{Native 3D} &
% \textbf{Open code} &
% \textbf{Data mixture} \\
% \midrule
% MedGemma & 416M & \n & \n & Mixture of radiology, pathology, dermatology, ophthalmology\\
% MedImageInsight & 362M & \n & \n & Mixture of radiology, pathology, dermatology, ophthalmology \\
% Lingshu & 676M & \n & \n & Mixture of radiology, pathology, dermatology, ophthalmology, endoscopy \\
% Merlin & 121M & \y & \y & 3D abdominal CT \\
% \midrule
% \textbf{\name(Ours)} & 79M & \y & \y & 3D CT and MR \\
% \bottomrule
% \end{tabularx}
% \end{table}


% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \begin{table}[t]
% \centering
% % \caption{Evaluation Frameworks}
% \label{tab:benchmark_characteristics}
% % \begin{tabularx}{\linewidth}{l *{5}{>{\centering\arraybackslash}X}}
% \begin{tabularx}{\linewidth}{p{0.2\linewidth} C{0.15\linewidth} C{0.33\linewidth} C{0.2\linewidth}}
% \toprule
% \textbf{Evaluation Framework} &
% \textbf{Image format} &
% \textbf{Task and label source} &
% \textbf{Extensibility} \\
% \midrule
% VQA-RAD & Single-slice JPEG & Medical student QA & \n\\
% SLAKE & Single slice JPG & Physician QA with knowledge graph-curated labels & \n \\
% PMC-VQA & Single-slice JPG & Medical figures and captions & \n \\
% OmniMedVQA & Single-slice PNG & Classification datasets & \n \\
% MMMU & Single-slice PNG & Textbooks, online resources & \n \\
% RadLE & Single slices & Radiologist-selected complex cases & \n \\
% MedXpertQA & Single-slice JPEG & Medical exams and textbooks & \n \\
% \midrule
% \textbf{RATE (Ours)} & \textbf{Full-resolution 3D DICOMs} & \textbf{Real-world radiology workflows} & \textbf{Can be extended to any new dataset} \\
% \bottomrule
% \end{tabularx}
% \end{table}
